Soliton trapping, transmission and wake in modulationally unstable media

Interactions between solitons and the coherent oscillation structures generated by localized disturbances via modulational instability are studied within the framework of the focusing nonlinear Schrodinger equation. Two main interaction regimes are identified based on the relative value of the velocity of the incident soliton compared to the amplitude of the background: soliton transmission and soliton trapping. Specifically, when the incident soliton velocity exceeds a certain threshold, the soliton passes through the coherent structure and emerges on the other side with its velocity unchanged. Conversely, when the incident soliton velocity is below the threshold, once the soliton enters the coherent structure, it remains confined there forever. It is demonstrated that the soliton is not destroyed, but its velocity inside the coherent structure is different from its initial one. Moreover, it is also shown that, depending on the location of the discrete eigenvalue associated to the soliton, these phenomena can also be accompanied by the generation of additional, localized propagating waves in the coherent structure, akin to a soliton-generated wake.

==> references.tex <==
\catcode`\@ 11
\def\d@mmyjournal{\errmessage{Reference foul up: nested \journal macros}}
\def\@biblabel#1{#1.}	
\begin{thebibliography}{OO}
\def\booktitle#1{\textit{#1}}
\itemsep 0pt

\kern-\medskipamount

\item[*] Electronic address: biondini@buffalo.edu.~\ 

\bibitem{ZO2009}
V. E. Zakharov and L. A. Ostrovsky, 
  \reftitle{Modulational instability: The beginning}, 
  \href{http://www.sciencedirect.com/science/article/pii/S0167278908004223}
  {Phys. D \textbf{238}, 540--548 (2009)}

\bibitem{DudleyTaylor}
J. M. Dudley and J. R. Taylor,
  \booktitle{Supercontinuum generation in optical fibers}
  (Cambridge University Press, 2010)

\bibitem{zakharov2009}
V. E. Zakharov,
  \reftitle{Turbulence in integrable systems},
  \href{\doibase 10.1111/j.1467-9590.2009.00430.x}
  {{{Stud. Appl. Math.}} \textbf{122},\ {219--234} (2009)}

\bibitem{randoux2014}
S. Randoux, P. Walczak, M. Onorato and P. Suret,
  \reftitle{Intermittency in integrable turbulence},
  \href{\doibase 10.1103/PhysRevLett.113.113902}
  {Phys. Rev. Lett. \textbf{113}, 113902 (2014)}

\bibitem{az2014}
D. S. Agafontsev and V. E. Zakharov, 
  \reftitle{Integrable turbulence and formation of rogue waves}, 
  \href{http://iopscience.iop.org/article/10.1088/0951-7715/28/8/2791/pdf}
  {Nonlinearity, \textbf{28}, 2791--2821 (2015)}

\bibitem{onoratoosborne}
M. Onorato, A. R. Osborne and M. Serio,
  \reftitle{Modulational instability in crossing sea states: A possible mechanism for the formation of freak waves},
  \href{\doibase 10.1103/PhysRevLett.96.014503}
  {Phys. Rev. Lett. \textbf{96}, 014503 (2006)}

\bibitem{solli}
D. R.  Solli, C. Ropers, P. Koonath  and B. Jalali,
  \reftitle{Optical rogue waves},
  \href{\doibase 10.1038/nature06402} 
  {{{Nature}} \textbf{450},\ {1054--1057} {(2007})}

\bibitem{naturephys}
B. Kibler \textit{et alii},
  %{{B. {Kibler}}, {J. {Fatome}}, {C. {Finot}}, {G. {Millot}}, {F. {Dias}}, {G. {Genty}}, {N. {Akhmediev}},\ and\ {{J.~M.}\ {Dudley}},}
  \reftitle{The {Peregrine} soliton in nonlinear fibre optics},
  \href{\doibase 10.1038/nphys1740} 
  {{Nature Phys.}\ \textbf{6},\  {790--795} (2010)}%

\bibitem{AS1981}
M. J. Ablowitz and H. Segur,
  \booktitle{Solitons and the inverse scattering transform}
  (SIAM, Philadelphia, 1981)

\bibitem{Agrawal2007}
  G. P. Agrawal,
  \booktitle{Nonlinear fiber optics}
  (Academic Press, New York, 2007)

\bibitem{IR2000}
I. Infeld and G. Rowlands, 
\booktitle{Nonlinear waves, solitons and chaos}
(Cambridge University Press, London, 2000) 

\bibitem{NMPZ1984}
S. P. Novikov, S. V. Manakov, L. P. Pitaevskii and V. E. Zakharov, 
\booktitle{Theory of solitons: The inverse scattering transform} 
(Plenum, 1984)

\bibitem{PS2003}
L. P. Pitaevskii and S. Stringari,
\booktitle{Bose-Einstein condensation},
(Clarendon Press, Oxford, 2003)

\bibitem{benjaminfeir}
T. B. Benjamin and J. E. Feir, 
\reftitle{The disintegration of wave trains on deep water}, 
J. Fluid Mech. \textbf{27}, 417  (1967)

\bibitem{zakharovgelash}
V. E. Zakharov and A. A. Gelash,
  \reftitle{Nonlinear stage of modulation instability},
  \href{\doibase 10.1103/PhysRevLett.111.054101}
  {{Phys. Rev. Lett.} \textbf{111}\, {054101} (2013)}

\bibitem{gelashzakharov}
A. A. Gelash and V. E. Zakharov, 
  \reftitle{Superregular solitonic solutions: a novel scenario for the nonlinear stage of modulation instability},
  \href{https://doi.org/10.1088/0951-7715/27/4/R1}
  {Nonlinearity \textbf{27}, 1 (2014)}

\bibitem{kibler}
B. Kibler, A. Chabchoub, A. Gelash, N. Akhmediev and V. E. Zakharov,
  \reftitle{Superregular breathers in optics and hydrodynamics: Omnipresent modulation instability beyond simple periodicity},
  \href{http://journals.aps.org/prx/pdf/10.1103/PhysRevX.5.041026}
  {Phys. Rev. X \textbf{5}, 041026 (2015)}

\bibitem{biondinifagerstrom}
G. Biondini and E. R. Fagerstrom, 
  \reftitle{The integrable nature of modulational instability},
  \href{\doibase 10.1137/140965089}
  {{{SIAM J. Appl.  Math.}} \textbf{75},\ {136--163} (2015)}

\bibitem{biondinimantzavinos}
G. Biondini and D. Mantzavinos,
  \reftitle{Universal nature of the nonlinear stage of modulational instability},
  \href{\doibase 10.1103/PhysRevLett.116.043902} 
  {{{Phys. Rev. Lett.}} \textbf{116},\ {043902} (2016)}%

\bibitem{CPAM2017}%
G. Biondini and D. Mantzavinos,
  \reftitle{Long-time asymptotics for the focusing nonlinear {Schr\"odinger} equation with nonzero boundary conditions at infinity and asymptotic stage of modulational instability},
  \href{\doibase 10.1002/cpa.21701}
  {Commun. Pure Appl. Math. \textbf{70}, {2300--2365} (2017)}

\bibitem{biondinilimantzavinos}
G.~Biondini, S.~Li and D.~Mantzavinos, 
  \reftitle{Oscillation structure of localized perturbations in modulationally unstable media}, 
  \href{\doibase 10.1103/PhysRevE.94.060201}
  {Phys. Rev. E \textbf{94}, 060201R (2016)}

\bibitem{SIREV}
G.~Biondini, S.~Li, D.~Mantzavinos and S. Trillo, 
  \reftitle{Universal behavior of modulationally unstable media},
  to appear in SIAM Rev.,
  \href{http://arxiv.org/pdf/1710.05068}
  {arXiv:1710.05068 [nlin.ps] (2017)}

\bibitem{ZS1972}
V. E. Zakharov and A. B. Shabat,
  \reftitle{Exact theory of two-dimensional self-focusing and one-dimensional self-modulation of waves in nonlinear media},
  Sov. Phys. JETP \textbf{34}, 62 (1972)

\bibitem{supplement}
Please see the Supplementary Material for further details.

\bibitem{biondinikovacic}
G. Biondini and G. Kova\v{c}i\v{c},
  \reftitle{Inverse scattering transform for the focusing nonlinear {Schr\"odinger} equation with nonzero boundary conditions},
  \href{http://scitation.aip.org/content/aip/journal/jmp/55/3/10.1063/1.4868483}
  {J. Math. Phys.\textbf{55}, 031506 (2014)}%

\bibitem{Gakhov}
F. D. Gakhov,
\booktitle{Boundary value problems}
(Pergamon Press, 1966)

\bibitem{TrogdonOlver}
T. Trogdon and S. Olver,
\booktitle{Riemann-Hilbert problems, their numerical solution, and the computation of nonlinear special functions}
(SIAM, Philadelphia, 2016)

\bibitem{whitham}
G. B. Whitham,
\textsl{Linear and nonlinear waves}
(Wiley, 1974)

%\bibitem{deiftzhou}
%P. Deift and X. Zhou,
%\reftitle{A steepest descent method for oscillatory Riemann-Hilbert problems. Asymptotics for the mKdV equation}, 
%\href{\doibase 10.2307/2946540}
%{Ann. Math. \textbf{137}, 295 (1993)}

\bibitem{dkkz1996}
P. Deift, S. Kamvissis, T. Kriecherbauer and X. Zhou, 
\reftitle{The Toda rarefaction problem}, 
\href{\doibase 10.1002/(SICI)1097-0312(199601)49:1<35::AID-CPA2>3.0.CO;2-8}
{Commun. Pure Appl. Math. \textbf{49}, 35-83 (1996)}

%\bibitem{m2008}
%P. D. Miller,
%\reftitle{Riemann-Hilbert problems with lots of discrete spectrum},
%{Contemp. Math. \textbf{458}, 163-181 (2008)}

\bibitem{trogdondeconinck}
T. Trogdon and B. Deconinck,
  \reftitle{A numerical dressing method for the nonlinear superposition of solutions of the KdV equation}, 
  \href{\doibase 10.1088/0951-7715/27/1/67}
  {Nonlinearity \textbf{27}, 67--85 (2013)}

\bibitem{LiBiondini}
S. Li and G. Biondini,
\reftitle{Soliton interactions and degenerate soliton complexes in modulationally unstable media},
%\href{***}
{to appear in EPJ Plus}

\bibitem{gelash}
A. A. Gelash,
  \reftitle{Formation of rogue waves from a locally perturbed condensate},
  \href{\doibase 10.1103/PhysRevE.97.022208}
  {Phys. Rev. E \textbf{97}, 022208 (2018)}

\bibitem{gordon}
J. P. Gordon,
\reftitle{Dispersive perturbations of solitons of the nonlinear Schr\"odinger equation},
  \href{https://doi.org/10.1364/JOSAB.9.000091}
  {J. Opt. Soc. Amer. B \textbf9, 91--97 (1992)}

\bibitem{kuznetsovmikhailov}
E. A. Kuznetsov, A. V. Mikhailov and I. A. Shimokhin,
  \reftitle{Nonlinear interaction of solitons and radiation},
  \href{https://doi.org/10.1016/0167-2789(95)00149-X}
  {Phys. D. \textbf{87}, 201--215 (1995)}
  
\bibitem{elhoefer}
G. A. El and M. A. Hoefer
  \reftitle{Dispersive shock waves and modulation theory},
  \href{https://doi.org/10.1016/j.physd.2016.04.006}
  {Phys. D \textbf{333}, 11--65 (2016)}

\bibitem{sprenger}
P. Sprenger, M. A. Hoefer and G. A. El,
  \reftitle{Hydrodynamic optical soliton tunneling},
  \href{http://arxiv.org/pdf/1711.05239}
  {arXiv:1711.05239 [nlin.ps] (2017)} 

\bibitem{maiden}
M. D. Maiden, D. V. Anderson, N. A. Franco, G. A. El and M. A. Hoefer
  \reftitle{Solitonic dispersive hydrodynamics: theory and observation},
  \href{http://arxiv.org/pdf/1711.01717}
   {arXiv:1711.01717 [nlin.ps] (2017)}
   
\bibitem{ablowitzluocole}
M. J. Ablowitz, X.-D.\ Luo and J. T. Cole
  \reftitle{Solitons, the Korteweg-deVries equation with step boundary values and pseudo-embedded eigenvalues},
  \href{https://arxiv.org/pdf/1802.03114.pdf}
   {arXiv:1802.03114 [nlin.si] (2018)}

\bibitem{BilmanMiller}
D. Bilman and P. D. Miller,
  \reftitle{A robust inverse scattering transform for the nonlinear Schrodinger equation}, 
  \href{https://arxiv.org/pdf/1710.06568}
  {arXiv:1710.06568 [nlin.si] (2017)}

\bibitem{el}
G.A. El, A.V. Gurevich, V.V. Khodorovskii and A.L. Krylov,
  \reftitle{Modulational instability and formation of a nonlinear oscillatory structure in a focusing medium},
  \href{\doibase 10.1016/0375-9601(93)90015-R}
  {{{Phys. Lett. A},} \textbf{177},\ {357--361} (1993)}

\bibitem{kamchatnov}
A.M. Kamchatnov,
\textit{Nonlinear periodic waves and their modulations}
(World Scientific, 2000)

\bibitem{NIST}
 {{F. W. Olver}, {D. W. Lozier}, {R. F. Boisvert} and {C. W. Clark}},
 \textit{NIST Handbook of Mathematical Functions},
 {(Cambridge University Press, 2010)}

\bibitem{yoshida}
H. Yoshida, 
  \reftitle{Construction of higher order symplectic integrators}, 
  \href{https://doi.org/10.1016/0375-9601(90)90092-3}
  {Phys. Lett. A \textbf{150}, 262 (1990)}

~

\end{thebibliography}

%A. Efimov, A. V. Yulin, D. V. Skryabin, J. C. Knight, N. Joly, F. G. Omenetto, A. J. Taylor, and P. Russell
%Interaction of an Optical Soliton with a Dispersive Wave
%Phys. Rev. Lett. 95, 213902 – Published 15 November 2005

%\bibitem{TrilloWabnitz}
%S. Trillo and S. Wabnitz,
%  \reftitle{{Dynamics of the nonlinear modulational instability in optical fibers},}
%  \href{\doibase 10.1364/OL.16.000986}
%  {{Opt. Lett.} \textbf{16}, {986--988} (1991)}

%\bibitem{kbk2015}
%D. K. Kraus, G. Biondini and G. Kova\v{c}i\v{c},
%  \reftitle{The focusing Manakov system with nonzero boundary conditions},
%\href{***}
%{\journal Nonlinearity &28, 3101 (2015)}

%\bibitem{Akhmediev2001}
% N. N. Akhmediev,
%\reftitle{Nonlinear physics: D\'ej\`a vu in optics},
%\href{\doibase 10.1038/35095154}
%{Nature \textbf{413}, 267--268 (2001)}

%\bibitem{garnier}
%J. Garnier and K. Kalimeris,
%\reftitle{Inverse scattering perturbation theory for the nonlinear Schr\"odinger equation with non-vanishing background},
%J. Phys. A \textbf{45}, 035202 (2012)

%\bibitem{ggkm1967}
%* C.S. Gardner, C.S. Greene, M.D. Kruskal and R.M. Miura, 
%\reftitle{Method for Solving the Korteweg-de Vries Equation}, 
%\journal Phys. Rev. Lett. &19, 1095 (1967)

%\bibitem{Trillo2}
%S. Trillo, S. Wabnitz and T.A.B. Kennedy,
%\reftitle{Nonlinear dynamics of dual-frequency-pumped multiwave mixing in optical fibers},
%Phys. Rev. A \textbf{50}, 1732 (1994)

%\bibitem{prl71p2683}
%M.J. Ablowitz, C.M. Schober and B.M. Herbst,
%\reftitle{Numerical chaos, roundoff errors and homoclinic manifolds},
%Phys. Rev. Lett. \textbf{71}, 2683 (1993)

%\bibitem{itskotlyarov}
%A.R. Its and V.P. Kotlyarov,
%  \reftitle{Explicit formulas for solutions of the NLS equation},
%  Dokl. Akad. Nauk Ukr. SSR A \textbf{11}, 965 (1965)

%\bibitem{maablowitz}
%Y.-C. Ma and M.J. Ablowitz, 
%  \reftitle{The periodic cubic NLS equation},
%  Stud. Appl. Math. \textbf{63}, 113 (1981)

%\bibitem{kuznetsov}
%E.A. Kuznetsov, 
%  \reftitle{Solitons in a parametrically unstable plasma}, 
%  Sov. Phys. Dokl. \textbf{22}, 507  (1977)

%\bibitem{ma}
%Y.-C. Ma, 
%  \reftitle{The Perturbed Plane-Wave Solutions of the Cubic {Schr\"{o}dinger} Equation},
%  \href{\doibase 10.1002/sapm197960143}
%  {Stud. Appl. Math. \textbf{60}, 43--58 (1979)}

%\bibitem{peregrine}
%D. H. Peregrine, 
%  \reftitle{Water waves, nonlinear Schr\"odinger equations and their solutions}, 
%  \href{\doibase 10.1017/S0334270000003891}
%  {Austral. Math. Soc. Ser. B \textbf{25}, 16--43 (1983)}

%\bibitem{akhmediev}
%N.N. Akhmediev and V.I. Korneev,
%   \reftitle{Modulational instability and periodic solutions of the nonlinear Schr\"odinger equation},
%   \href{\doibase 10.1007/BF01037866}
%   {Theor. Math. Phys. \textbf{69}, 1089--1093 (1986)}

%\bibitem{tajiriwatanabe}
%M. Tajiri and Y. Watanabe, 
%  \reftitle{Breather solutions to the focusing nonlinear Schr\"odinger equation}, 
%  \href{\doibase 10.1103/PhysRevE.57.3510}
%  {Phys. Rev. E \textbf{57}, 3510--3519 (1998)}

%\bibitem{zakharovshabat1973}
%V.E. Zakharov and A.B. Shabat,
%\reftitle{Interaction between solitons in a stable medium},
%\journal Sov. Phys. JETP &37, 823 (1973)



